SN 2021adxl: A luminous nearby interacting supernova in an extremely low metallicity environment

SN 2021adxl is a slowly evolving, luminous, Type IIn supernova with asymmetric emission line profiles, similar to the well-studied SN 2010jl. We present extensive optical, near-ultraviolet, and near-infrared photometry and spectroscopy covering ~1.5 years post discovery. SN 2021adxl occurred in an unusual environment, atop a vigorously star-forming region that is offset from its host galaxy core. The appearance of Ly-alpha, O II, as well as the compact core, would classify the host of SN 2021adxl as a Blueberry galaxy, analogous to the higher redshift Green Pea galaxies. Using several abundance indicators, we find a metallicity of the explosion environment of only 10% solar, the lowest reported metallicity for a Type IIn SN environment. SN 2021adxl reaches a peak magnitude of r ~ -20.2 mag and since discovery, SN 2021adxl has faded by only ~4 magnitudes in the r band with a cumulative radiated energy of ~1.5e50 erg over 18 months. SN 2021adxl shows strong signs of interaction with a complex circumstellar medium, seen by the detection of X-rays, revealed by the detection of coronal emission lines, and through multi-component hydrogen and helium profiles. In order to further understand this interaction, we model the H{\alpha} profile using a Monte-Carlo electron scattering code. The blueshifted high-velocity component is consistent with emission from a radially thin, spherical shell resulting in the broad emission components due to electron scattering. Using the velocity evolution of this emitting shell, we find that the SN ejecta collide with circumstellar material of at least 5 Msun, assuming a steady-state mass-loss rate of 4-6e-3 Msun per year for the first ~200 days of evolution. Continuing the observations of SN 2021adxl may reveal signatures of dust formation or an infrared excess, similar to that seen for SN 2010jl.

==> tables/SN2021adxl_lineflux.tex <==
\begin{table*}
\centering
\caption{Measured parameters for several emission lines in the VLT/XShooter spectrum taken on 2023-02-26 (+480d). Flux has been corrected for MW extinction. Errors for each measurement are given in parentheses. Errors on the Equivalent Width (EW) are 
from %given by Eq. 6 from 
\citet[][their Eq. 6]{Cayrel1988}. Note for the Hydrogen emission lines, we measure the flux from the narrow component only.}
\label{tab:lineflux}
\begin{tabular}{l|ccr}
\toprule
 & Flux [$ { \rm erg~s^{-1}~cm^{-2} }$] & FWHM [$ { \rm km~s^{-1}] }$  & EW [$ { \rm \AA] }$  \\
\midrule
$ {\rm H~\lambda4340 }$ & 3.834 (0.020) $\times 10^{-16}$ & 36.408 (0.164) & -12.790 (0.003) \\
$ {\rm H~\lambda4861 }$ & 8.351 (0.019) $\times 10^{-16}$ & 37.061 (0.156) & -19.417 (0.002) \\
$ {\rm H~\lambda6563 }$ & 2.047 (0.005) $\times 10^{-15}$ & 27.633 (0.182) & -14.439 (0.001) \\
$ {\rm [Ar~III]~\lambda7135 }$ & 2.246 (0.093) $\times 10^{-17}$ & 20.292 (0.332) & -2.494 (0.028) \\
$ {\rm [N~II]~\lambda6583 }$ & 1.495 (0.245) $\times 10^{-17}$ & 19.677 (0.626) & -0.159 (0.109) \\
$ {\rm [O~III]~\lambda4363 }$ & 6.503 (0.199) $\times 10^{-17}$ & 34.855 (0.327) & -2.242 (0.020) \\
$ {\rm [O~III]~\lambda5007 }$ & 3.079 (0.005) $\times 10^{-15}$ & 34.975 (0.202) & -139.444 (0.001) \\
$ {\rm [O~II]~\lambda3726 }$ & 4.396 (0.043) $\times 10^{-16}$ & 37.360 (0.158) & -13.415 (0.006) \\
$ {\rm [O~II]~\lambda3729 }$ & 6.253 (0.087) $\times 10^{-16}$ & 35.613 (0.209) & -19.163 (0.009) \\
$ {\rm [S~ III]~\lambda9069 }$ & 5.686 (0.095) $\times 10^{-17}$ & 22.275 (0.157) & -8.518 (0.011) \\
$ {\rm [S~ II]~\lambda6716 }$ & 7.301 (0.119) $\times 10^{-17}$ & 24.933 (0.558) & -6.277 (0.011) \\
$ {\rm [S~II]~\lambda6731 }$ & 5.263 (0.102) $\times 10^{-17}$ & 24.194 (0.472) & -4.766 (0.013) \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/SN2021adxl_metallicity.tex <==
\begin{table}
\centering
\caption{Metallicity measurements for \xdos using verious abundance indictures found in literature.}
\label{tab:metallicty}
\begin{tabular}{lccc}
\toprule
 & $ { \rm 12 + log(O/H) } $ & $ {\rm Z/Z_{\odot}}$ \\
\midrule
PyNeb & 7.61 & 0.08 \\
N2 & 7.76 & 0.12 \\
O3N2 & 7.95 & 0.18 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/observation_log.tex <==
\begin{table*}
\centering
\caption{Spectropscopy log for \xdos. Phase with reference to discovery date [MJD 59521]}
\label{tab:observation_log}
\begin{tabular}{ccccccc}
\toprule
Date & MJD & Phase (d) & Telescope & Instrument & Resolution ($\lambda / \Delta \lambda $) & Exposure Time (s) \\
\midrule
2021-11-09 & 59527 & +6 & P60 & SEDM IFU & 100 & 2400 \\
2022-02-02 & 59612 & +91 & P200 & DBSP & 4000 & 300 \\
2022-02-03 & 59613 & +92 & P60 & SEDM IFU & 100 & 2400 \\
2022-02-04 & 59614 & +93 & P60 & SEDM IFU & 100 & 2400 \\
2022-02-05 & 59615 & +94 & Keck & LRIS  & 300-5000 & 2400 \\
2022-02-05 & 59615 & +94 & P60 & SEDM IFU & 100 & 2400 \\
2022-02-06 & 59616 & +95 & P60 & SEDM IFU & 100 & 2400 \\
2022-02-07 & 59617 & +96 & P60 & SEDM IFU & 100 & 2400 \\
2022-02-09 & 59619 & +98 & P60 & SEDM IFU & 100 & 2400 \\
2022-02-10 & 59620 & +99 & P60 & SEDM IFU & 100 & 2400 \\
2022-02-11 & 59621 & +100 & P60 & SEDM IFU & 100 & 2400 \\
2022-02-14 & 59624 & +103 & NOT & ALFOSC+Grism4 & 360 & 1800 \\
2022-02-20 & 59630 & +109 & P60 & SEDM IFU & 100 & 2400 \\
2022-02-26 & 59636 & +115 & VLT & X-shooter & 5400/8900/5600 & 2400/2458/2400 \\
2022-02-26 & 59636 & +115 & P60 & SEDM IFU & 100 & 2400 \\
2022-03-02 & 59640 & +119 & P60 & SEDM IFU & 100 & 2160 \\
2022-03-09 & 59647 & +126 & P60 & SEDM IFU & 100 & 2400 \\
2022-03-14 & 59652 & +131 & P60 & SEDM IFU & 100 & 2400 \\
2022-03-21 & 59659 & +138 & P60 & SEDM IFU & 100 & 2400 \\
2022-03-21 & 59659 & +138 & P60 & SEDM IFU & 100 & 2400 \\
2022-03-23 & 59661 & +140 & P60 & SEDM IFU & 100 & 2400 \\
2022-03-23 & 59661 & +140 & P60 & SEDM IFU & 100 & 2400 \\
2022-03-28 & 59666 & +145 & P60 & SEDM IFU & 100 & 2400 \\
2022-03-30 & 59668 & +147 & NOT & ALFOSC+Grism4 & 360 & 1800 \\
2022-04-01 & 59670 & +149 & P60 & SEDM IFU & 100 & 2400 \\
2022-04-11 & 59680 & +159 & HST & COS/STIS & 2000-3000 & 1911 \\
2022-04-11 & 59680 & +159 & P60 & SEDM IFU & 100 & 2400 \\
2022-04-18 & 59687 & +166 & P60 & SEDM IFU & 100 & 2160 \\
2022-04-26 & 59695 & +174 & NOT & ALFOSC+ Grism4 & 360 & 1800 \\
2022-05-02 & 59701 & +180 & VLT & X-shooter & 5400/8900/5600 & 3600 \\
2022-05-15 & 59714 & +193 & P60 & SEDM IFU & 100 & 2160 \\
2022-05-27 & 59726 & +205 & NOT & ALFOSC+Grism4 & 360 & 1800 \\
2022-06-12 & 59742 & +221 & P60 & SEDM IFU & 100 & 2160 \\
2022-11-09 & 59892 & +371 & P60 & SEDM IFU & 100 & 2400 \\
2022-11-25 & 59908 & +387 & NOT & ALFOSC+Grism4 & 360 & 1200 \\
2022-12-08 & 59921 & +400 & P60 & SEDM IFU & 100 & 1800 \\
2023-01-18 & 59962 & +441 & VLT & X-shooter & 5400/8900/5600 & 1800/1860/1800 \\
2023-02-26 & 60001 & +480 & VLT & X-shooter & 5400/8900/5600 & 3600/3716/3600 \\
2023-03-23 & 60026 & +505 & NOT & ALFOSC+Grism4 & 360 & 3300 \\
2023-04-16 & 60050 & +529 & NOT & ALFOSC+Grism4 & 360 & 3300 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/photometry_tables.tex <==
\begin{table}
\centering
\caption{Photometry values and uncertainties for \xdos.}
\label{tab:photomery}
\begin{tabular}{rrrl}
\toprule
mjd & mag & error & filter \\
\midrule
59526.530 & 14.323 & 0.027 & r \\
59526.530 & 14.323 & 0.027 & r \\
59526.530 & 14.323 & 0.027 & r \\
59526.530 & 14.322 & 0.003 & r \\
59526.532 & 14.337 & 0.024 & r \\
59526.532 & 14.337 & 0.024 & r \\
59526.532 & 14.331 & 0.003 & r \\
59526.532 & 14.337 & 0.024 & r \\
59526.535 & 14.332 & 0.003 & r \\
59526.535 & 14.332 & 0.027 & r \\
59526.535 & 14.332 & 0.027 & r \\
59526.535 & 14.332 & 0.027 & r \\
59526.537 & 14.353 & 0.020 & r \\
59526.537 & 14.387 & 0.003 & r \\
59526.537 & 14.353 & 0.020 & r \\
59526.537 & 14.353 & 0.020 & r \\
59526.540 & 14.352 & 0.003 & r \\
59526.540 & 14.339 & 0.022 & r \\
59526.540 & 14.339 & 0.022 & r \\
59526.540 & 14.339 & 0.022 & r \\
59527.518 & 14.362 & 0.036 & r \\
59527.532 & 14.343 & 0.003 & r \\
59527.532 & 14.333 & 0.020 & r \\
59527.532 & 14.333 & 0.020 & r \\
59527.532 & 14.333 & 0.020 & r \\
59527.534 & 14.318 & 0.003 & r \\
59527.534 & 14.316 & 0.027 & r \\
59527.534 & 14.316 & 0.027 & r \\
59527.534 & 14.316 & 0.027 & r \\
59527.537 & 14.311 & 0.030 & r \\
59527.537 & 14.311 & 0.030 & r \\
59527.537 & 14.311 & 0.030 & r \\
59527.537 & 14.335 & 0.003 & r \\
59527.539 & 14.350 & 0.003 & r \\
59527.539 & 14.355 & 0.019 & r \\
59527.539 & 14.355 & 0.019 & r \\
59527.539 & 14.355 & 0.019 & r \\
59527.542 & 14.374 & 0.003 & r \\
59527.542 & 14.351 & 0.018 & r \\
59527.542 & 14.351 & 0.018 & r \\
59527.542 & 14.351 & 0.018 & r \\
59528.532 & 14.343 & 0.019 & r \\
59528.532 & 14.343 & 0.019 & r \\
59528.532 & 14.343 & 0.019 & r \\
59528.532 & 14.402 & 0.003 & r \\
59528.535 & 14.386 & 0.020 & r \\
59528.535 & 14.445 & 0.003 & r \\
59528.535 & 14.386 & 0.020 & r \\
59528.535 & 14.386 & 0.020 & r \\
59528.537 & 14.358 & 0.019 & r \\
59528.537 & 14.358 & 0.019 & r \\
59528.537 & 14.358 & 0.019 & r \\
59528.537 & 14.425 & 0.003 & r \\
59528.542 & 14.337 & 0.015 & r \\
59528.542 & 14.337 & 0.015 & r \\
59528.542 & 14.394 & 0.003 & r \\
59528.542 & 14.337 & 0.015 & r \\
59528.546 & 14.334 & 0.023 & r \\
59528.546 & 14.400 & 0.003 & r \\
59528.546 & 14.334 & 0.023 & r \\
59528.546 & 14.334 & 0.023 & r \\
59531.522 & 14.523 & 0.004 & i \\
59550.505 & 14.405 & 0.003 & r \\
59550.505 & 14.427 & 0.026 & r \\
59550.505 & 14.427 & 0.026 & r \\
59552.552 & 13.980 & 0.260 & J \\
59604.425 & 13.950 & 0.180 & J \\
59607.456 & 13.900 & 0.100 & J \\
59610.451 & 14.100 & 0.160 & J \\
59613.465 & 13.850 & 0.110 & J \\
59613.471 & 14.827 & 0.041 & r \\
59613.473 & 14.814 & 0.032 & i \\
59614.324 & 14.818 & 0.031 & i \\
59614.382 & 14.819 & 0.038 & r \\
59614.384 & 14.803 & 0.030 & i \\
59615.346 & 14.831 & 0.111 & r \\
59615.375 & 14.803 & 0.028 & r \\
59615.376 & 14.812 & 0.023 & r \\
59615.382 & 14.784 & 0.019 & i \\
59615.384 & 14.794 & 0.024 & i \\
59615.466 & 13.930 & 0.110 & J \\
59616.280 & 14.798 & 0.052 & r \\
59616.298 & 14.808 & 0.028 & i \\
59616.327 & 14.846 & 0.061 & r \\
59616.356 & 14.820 & 0.042 & r \\
59616.360 & 14.815 & 0.027 & i \\
59617.320 & 14.841 & 0.034 & i \\
59617.459 & 13.970 & 0.140 & J \\
59618.330 & 14.828 & 0.025 & r \\
59618.332 & 14.790 & 0.022 & i \\
59619.083 & 15.402 & 0.043 & g \\
59619.084 & 14.883 & 0.033 & r \\
59619.288 & 14.872 & 0.033 & r \\
59619.317 & 14.851 & 0.025 & r \\
59619.327 & 14.827 & 0.023 & i \\
59619.456 & 14.070 & 0.110 & J \\
59620.292 & 14.876 & 0.042 & r \\
59620.302 & 14.810 & 0.027 & i \\
59621.260 & 14.962 & 0.040 & r \\
59621.291 & 14.850 & 0.029 & r \\
59621.293 & 14.806 & 0.019 & i \\
59622.440 & 14.926 & 0.033 & r \\
59622.440 & 14.926 & 0.033 & r \\
59622.440 & 14.969 & 0.004 & r \\
59622.440 & 14.926 & 0.033 & r \\
59622.502 & 15.413 & 0.032 & g \\
59622.502 & 15.413 & 0.032 & g \\
59622.502 & 15.465 & 0.005 & g \\
59622.502 & 15.413 & 0.032 & g \\
59623.053 & 15.432 & 0.038 & g \\
59623.053 & 14.899 & 0.050 & r \\
59623.054 & 14.914 & 0.034 & i \\
59623.054 & 14.831 & 0.057 & z \\
59624.394 & 14.843 & 0.032 & r \\
59624.394 & 14.833 & 0.003 & r \\
59624.394 & 14.843 & 0.032 & r \\
59624.394 & 14.843 & 0.032 & r \\
59624.441 & 15.098 & 0.005 & i \\
59624.506 & 15.448 & 0.028 & g \\
59624.506 & 15.472 & 0.006 & g \\
59624.506 & 15.448 & 0.028 & g \\
59624.506 & 15.448 & 0.028 & g \\
59627.032 & 15.479 & 0.052 & g \\
59627.441 & 15.527 & 0.031 & g \\
59627.441 & 15.527 & 0.031 & g \\
59627.441 & 15.527 & 0.031 & g \\
59627.441 & 15.636 & 0.016 & g \\
59630.333 & 14.925 & 0.020 & r \\
59630.334 & 14.897 & 0.033 & r \\
59630.334 & 14.897 & 0.033 & r \\
59630.334 & 14.860 & 0.004 & r \\
59630.334 & 14.897 & 0.033 & r \\
59630.368 & 14.938 & 0.018 & r \\
59630.370 & 14.916 & 0.018 & i \\
59630.380 & 15.502 & 0.005 & g \\
59630.380 & 15.518 & 0.028 & g \\
59630.380 & 15.518 & 0.028 & g \\
59630.380 & 15.518 & 0.028 & g \\
59633.704 & 17.208 & 0.057 & UVW1 \\
59633.705 & 16.453 & 0.059 & U \\
59633.706 & 15.672 & 0.051 & B \\
59633.707 & 17.727 & 0.054 & UVW2 \\
59633.708 & 15.248 & 0.067 & V \\
59633.710 & 17.680 & 0.055 & UVM2 \\
59636.261 & 14.962 & 0.024 & r \\
59636.296 & 14.999 & 0.020 & r \\
59636.298 & 14.959 & 0.017 & i \\
59637.319 & 14.957 & 0.029 & r \\
59637.319 & 14.957 & 0.029 & r \\
59637.319 & 14.982 & 0.004 & r \\
59637.319 & 14.957 & 0.029 & r \\
59638.483 & 17.468 & 0.057 & UVW1 \\
59638.484 & 16.673 & 0.058 & U \\
59638.485 & 15.755 & 0.048 & B \\
59638.486 & 17.785 & 0.050 & UVW2 \\
59638.488 & 15.322 & 0.063 & V \\
59638.490 & 17.642 & 0.052 & UVM2 \\
59639.338 & 15.696 & 0.006 & g \\
59639.338 & 15.614 & 0.037 & g \\
59639.338 & 15.614 & 0.037 & g \\
59640.491 & 15.007 & 0.032 & r \\
59640.517 & 15.002 & 0.027 & r \\
59640.523 & 14.956 & 0.021 & i \\
59647.490 & 15.068 & 0.034 & r \\
59647.521 & 15.042 & 0.031 & r \\
59647.523 & 15.090 & 0.026 & i \\
59652.176 & 15.073 & 0.033 & r \\
59652.211 & 15.108 & 0.039 & r \\
59652.213 & 15.141 & 0.027 & i \\
59659.197 & 15.173 & 0.037 & r \\
59659.230 & 15.256 & 0.026 & i \\
59659.232 & 15.175 & 0.037 & r \\
59659.265 & 15.241 & 0.033 & i \\
59659.995 & 17.455 & 0.073 & UVW1 \\
59659.995 & 17.456 & 0.073 & UVW1 \\
59659.996 & 16.841 & 0.080 & U \\
59659.996 & 16.834 & 0.080 & U \\
59659.996 & 16.058 & 0.070 & B \\
59659.996 & 16.064 & 0.070 & B \\
59659.997 & 17.957 & 0.069 & UVW2 \\
59659.997 & 17.968 & 0.069 & UVW2 \\
59659.998 & 15.735 & 0.098 & V \\
59659.998 & 15.733 & 0.098 & V \\
59659.999 & 17.897 & 0.076 & UVM2 \\
59659.999 & 17.899 & 0.076 & UVM2 \\
59661.153 & 15.151 & 0.031 & r \\
59661.184 & 15.160 & 0.019 & r \\
59661.186 & 15.198 & 0.017 & i \\
59661.188 & 15.158 & 0.026 & r \\
59661.220 & 15.149 & 0.032 & r \\
59661.224 & 15.187 & 0.019 & i \\
59666.291 & 15.212 & 0.031 & r \\
59667.946 & 17.526 & 0.061 & UVW1 \\
59667.947 & 16.771 & 0.063 & U \\
59667.948 & 16.134 & 0.058 & B \\
59667.951 & 15.548 & 0.072 & V \\
59671.384 & 15.225 & 0.009 & r \\
59671.386 & 15.286 & 0.013 & i \\
59671.398 & 15.982 & 0.006 & g \\
59671.398 & 16.022 & 0.024 & g \\
59671.398 & 16.022 & 0.024 & g \\
59671.398 & 16.022 & 0.024 & g \\
59671.398 & 15.990 & 0.025 & g \\
59671.398 & 15.990 & 0.025 & g \\
59671.829 & 17.537 & 0.057 & UVW1 \\
59671.830 & 16.871 & 0.062 & U \\
59671.830 & 16.099 & 0.054 & B \\
59671.831 & 17.809 & 0.050 & UVW2 \\
59671.832 & 15.576 & 0.068 & V \\
59671.833 & 17.780 & 0.064 & UVM2 \\
59673.280 & 15.311 & 0.040 & i \\
59673.280 & 15.311 & 0.040 & i \\
59673.280 & 15.573 & 0.007 & i \\
59674.300 & 15.209 & 0.004 & r \\
59674.300 & 15.231 & 0.026 & r \\
59674.300 & 15.231 & 0.026 & r \\
59674.300 & 15.231 & 0.026 & r \\
59675.586 & 17.550 & 0.076 & UVW1 \\
59675.586 & 17.081 & 0.089 & U \\
59675.586 & 16.363 & 0.079 & B \\
59675.588 & 17.930 & 0.068 & UVW2 \\
59675.588 & 15.818 & 0.101 & V \\
59675.590 & 17.835 & 0.066 & UVM2 \\
59676.277 & 14.350 & 0.260 & J \\
59676.337 & 15.364 & 0.006 & r \\
59676.337 & 15.299 & 0.026 & r \\
59676.337 & 15.299 & 0.026 & r \\
59677.910 & 16.027 & 0.031 & g \\
59677.910 & 15.256 & 0.048 & r \\
59677.911 & 15.463 & 0.051 & i \\
59677.911 & 15.301 & 0.072 & z \\
59678.253 & 15.196 & 0.004 & r \\
59678.253 & 15.259 & 0.032 & r \\
59678.253 & 15.260 & 0.032 & r \\
59678.253 & 15.260 & 0.032 & r \\
59678.316 & 16.030 & 0.030 & g \\
59678.316 & 16.030 & 0.030 & g \\
59678.316 & 16.011 & 0.006 & g \\
59678.316 & 16.030 & 0.030 & g \\
59679.179 & 15.693 & 0.036 & i \\
59679.179 & 15.413 & 0.030 & i \\
59679.179 & 15.413 & 0.030 & i \\
59679.179 & 15.413 & 0.030 & i \\
59679.179 & 15.693 & 0.036 & i \\
59679.179 & 15.668 & 0.008 & i \\
59679.264 & 14.340 & 0.230 & J \\
59680.208 & 15.304 & 0.049 & r \\
59680.241 & 15.438 & 0.038 & i \\
59680.288 & 14.490 & 0.340 & J \\
59680.333 & 16.063 & 0.032 & g \\
59680.333 & 16.063 & 0.032 & g \\
59680.333 & 16.063 & 0.032 & g \\
59680.333 & 16.135 & 0.011 & g \\
59680.545 & 17.549 & 0.046 & UVW1 \\
59680.547 & 16.978 & 0.051 & U \\
59680.548 & 16.120 & 0.043 & B \\
59680.551 & 17.897 & 0.041 & UVW2 \\
59680.554 & 15.740 & 0.057 & V \\
59680.559 & 17.880 & 0.042 & UVM2 \\
59685.252 & 15.296 & 0.006 & r \\
59685.252 & 15.320 & 0.024 & r \\
59685.252 & 15.320 & 0.024 & r \\
59685.252 & 15.320 & 0.024 & r \\
59685.293 & 15.481 & 0.029 & i \\
59685.293 & 15.776 & 0.034 & i \\
59685.293 & 15.481 & 0.029 & i \\
59685.293 & 15.776 & 0.034 & i \\
59685.293 & 15.798 & 0.014 & i \\
59685.315 & 16.088 & 0.036 & g \\
59685.315 & 16.157 & 0.020 & g \\
59685.315 & 16.088 & 0.036 & g \\
59685.315 & 16.088 & 0.036 & g \\
59685.618 & 17.550 & 0.045 & UVW1 \\
59685.619 & 17.050 & 0.051 & U \\
59685.620 & 16.162 & 0.043 & B \\
59685.622 & 17.891 & 0.040 & UVW2 \\
59685.623 & 15.728 & 0.056 & V \\
59685.625 & 17.930 & 0.043 & UVM2 \\
59687.224 & 15.343 & 0.028 & r \\
59687.252 & 15.354 & 0.025 & r \\
59687.254 & 15.394 & 0.019 & i \\
59689.293 & 16.119 & 0.038 & g \\
59689.293 & 16.189 & 0.010 & g \\
59689.293 & 16.119 & 0.038 & g \\
59689.293 & 16.119 & 0.038 & g \\
59690.265 & 14.290 & 0.270 & J \\
59693.252 & 15.372 & 0.005 & r \\
59693.252 & 15.343 & 0.031 & r \\
59693.252 & 15.343 & 0.031 & r \\
59693.252 & 15.343 & 0.031 & r \\
59694.209 & 15.878 & 0.041 & i \\
59694.209 & 15.878 & 0.041 & i \\
59694.209 & 15.878 & 0.041 & i \\
59694.209 & 15.842 & 0.008 & i \\
59694.261 & 14.370 & 0.200 & J \\
59695.232 & 15.393 & 0.026 & r \\
59695.232 & 15.355 & 0.007 & r \\
59695.232 & 15.393 & 0.026 & r \\
59695.232 & 15.393 & 0.026 & r \\
59697.211 & 16.222 & 0.007 & g \\
59697.211 & 16.201 & 0.033 & g \\
59697.211 & 16.201 & 0.033 & g \\
59697.211 & 16.201 & 0.033 & g \\
59697.231 & 15.862 & 0.008 & i \\
59697.231 & 15.881 & 0.057 & i \\
59697.231 & 15.881 & 0.057 & i \\
59697.231 & 15.881 & 0.057 & i \\
59697.260 & 14.480 & 0.180 & J \\
59699.210 & 16.216 & 0.034 & g \\
59699.210 & 16.216 & 0.034 & g \\
59699.210 & 16.216 & 0.034 & g \\
59699.210 & 16.205 & 0.007 & g \\
59699.256 & 15.342 & 0.004 & r \\
59699.256 & 15.371 & 0.042 & r \\
59699.256 & 15.371 & 0.042 & r \\
59699.256 & 15.371 & 0.042 & r \\
59701.244 & 14.420 & 0.240 & J \\
59701.248 & 15.943 & 0.046 & i \\
59701.248 & 15.943 & 0.046 & i \\
59701.248 & 15.976 & 0.010 & i \\
59701.255 & 16.241 & 0.035 & g \\
59701.255 & 16.241 & 0.035 & g \\
59701.255 & 16.270 & 0.007 & g \\
59704.244 & 14.360 & 0.180 & J \\
59706.244 & 14.380 & 0.170 & J \\
59707.170 & 15.391 & 0.035 & r \\
59707.170 & 15.391 & 0.035 & r \\
59707.170 & 15.391 & 0.035 & r \\
59707.170 & 15.431 & 0.005 & r \\
59707.198 & 15.411 & 0.024 & r \\
59707.198 & 15.411 & 0.024 & r \\
59707.198 & 15.411 & 0.024 & r \\
59707.198 & 15.471 & 0.005 & r \\
59709.171 & 15.455 & 0.005 & r \\
59709.171 & 15.420 & 0.032 & r \\
59709.171 & 15.420 & 0.032 & r \\
59709.234 & 15.419 & 0.025 & r \\
59709.234 & 15.419 & 0.025 & r \\
59709.234 & 15.411 & 0.005 & r \\
59713.192 & 16.386 & 0.014 & g \\
59713.192 & 16.380 & 0.035 & g \\
59713.192 & 16.380 & 0.035 & g \\
59713.192 & 16.380 & 0.035 & g \\
59713.233 & 15.438 & 0.006 & r \\
59713.233 & 15.464 & 0.026 & r \\
59713.233 & 15.464 & 0.026 & r \\
59713.233 & 15.464 & 0.026 & r \\
59714.268 & 15.408 & 0.032 & r \\
59714.296 & 15.455 & 0.053 & r \\
59714.297 & 15.689 & 0.035 & i \\
59715.174 & 15.434 & 0.004 & r \\
59715.174 & 15.455 & 0.030 & r \\
59715.174 & 15.455 & 0.030 & r \\
59715.174 & 15.455 & 0.030 & r \\
59715.255 & 16.371 & 0.035 & g \\
59715.255 & 16.371 & 0.035 & g \\
59715.255 & 16.371 & 0.035 & g \\
59715.255 & 16.380 & 0.014 & g \\
59719.175 & 15.482 & 0.005 & r \\
59719.175 & 15.472 & 0.027 & r \\
59719.175 & 15.472 & 0.027 & r \\
59719.175 & 15.472 & 0.027 & r \\
59722.192 & 16.430 & 0.007 & g \\
59722.255 & 16.413 & 0.008 & g \\
59722.255 & 16.397 & 0.043 & g \\
59722.255 & 16.397 & 0.043 & g \\
59722.255 & 16.397 & 0.043 & g \\
59724.191 & 16.418 & 0.008 & g \\
59724.191 & 16.405 & 0.032 & g \\
59724.191 & 16.405 & 0.032 & g \\
59724.191 & 16.405 & 0.032 & g \\
59724.232 & 15.486 & 0.036 & r \\
59724.232 & 15.486 & 0.036 & r \\
59724.232 & 15.464 & 0.005 & r \\
59724.232 & 15.486 & 0.036 & r \\
59726.179 & 15.445 & 0.004 & r \\
59726.179 & 15.500 & 0.034 & r \\
59726.179 & 15.500 & 0.034 & r \\
59726.179 & 15.500 & 0.034 & r \\
59726.212 & 16.424 & 0.028 & g \\
59726.212 & 16.421 & 0.007 & g \\
59726.212 & 16.424 & 0.028 & g \\
59726.212 & 16.424 & 0.028 & g \\
59731.232 & 15.521 & 0.029 & r \\
59731.232 & 15.521 & 0.029 & r \\
59731.232 & 15.536 & 0.005 & r \\
59731.232 & 15.521 & 0.029 & r \\
59733.227 & 15.539 & 0.026 & r \\
59733.227 & 15.539 & 0.026 & r \\
59733.227 & 15.548 & 0.005 & r \\
59733.227 & 15.539 & 0.026 & r \\
59734.180 & 15.516 & 0.033 & r \\
59734.209 & 15.541 & 0.020 & r \\
59734.211 & 15.803 & 0.027 & i \\
59735.237 & 15.530 & 0.032 & r \\
59735.237 & 15.530 & 0.032 & r \\
59735.237 & 15.509 & 0.005 & r \\
59735.237 & 15.530 & 0.032 & r \\
59737.187 & 16.503 & 0.035 & g \\
59737.187 & 16.503 & 0.035 & g \\
59737.187 & 16.503 & 0.035 & g \\
59737.187 & 16.523 & 0.009 & g \\
59737.213 & 15.580 & 0.033 & r \\
59737.213 & 15.590 & 0.005 & r \\
59737.213 & 15.580 & 0.033 & r \\
59737.213 & 15.580 & 0.033 & r \\
59742.195 & 16.384 & 0.016 & i \\
59742.195 & 16.405 & 0.058 & i \\
59742.195 & 16.405 & 0.058 & i \\
59742.210 & 15.512 & 0.038 & r \\
59742.240 & 15.836 & 0.033 & i \\
59748.195 & 16.473 & 0.050 & i \\
59748.195 & 16.498 & 0.015 & i \\
59756.180 & 15.681 & 0.096 & r \\
59756.204 & 15.668 & 0.042 & r \\
59756.206 & 15.953 & 0.040 & i \\
59884.540 & 16.586 & 0.012 & r \\
59884.540 & 16.610 & 0.035 & r \\
59884.540 & 16.610 & 0.035 & r \\
59884.543 & 16.698 & 0.038 & r \\
59884.543 & 16.689 & 0.017 & r \\
59884.543 & 16.698 & 0.038 & r \\
59884.545 & 16.730 & 0.033 & r \\
59884.545 & 16.736 & 0.023 & r \\
59884.545 & 16.730 & 0.033 & r \\
59884.547 & 16.555 & 0.016 & r \\
59884.547 & 16.556 & 0.038 & r \\
59884.547 & 16.556 & 0.038 & r \\
59893.530 & 16.800 & 0.056 & r \\
59893.530 & 16.800 & 0.056 & r \\
59893.530 & 16.910 & 0.030 & r \\
59893.533 & 16.886 & 0.033 & r \\
59893.533 & 16.753 & 0.055 & r \\
59893.533 & 16.753 & 0.055 & r \\
59893.535 & 16.660 & 0.055 & r \\
59893.535 & 16.767 & 0.023 & r \\
59893.535 & 16.660 & 0.055 & r \\
59893.538 & 16.733 & 0.041 & r \\
59893.538 & 16.830 & 0.024 & r \\
59893.538 & 16.733 & 0.041 & r \\
59893.541 & 16.680 & 0.052 & r \\
59893.541 & 16.770 & 0.026 & r \\
59893.541 & 16.680 & 0.052 & r \\
59901.503 & 16.793 & 0.029 & r \\
59901.505 & 17.497 & 0.040 & i \\
59903.513 & 16.828 & 0.040 & r \\
59903.517 & 17.711 & 0.065 & i \\
59906.498 & 16.865 & 0.096 & r \\
59906.520 & 16.823 & 0.032 & r \\
59906.525 & 17.513 & 0.041 & i \\
59909.504 & 18.124 & 0.094 & g \\
59909.504 & 18.175 & 0.032 & g \\
59909.504 & 18.124 & 0.094 & g \\
59914.498 & 18.058 & 0.086 & g \\
59914.498 & 18.058 & 0.086 & g \\
59914.498 & 18.166 & 0.042 & g \\
59921.528 & 17.068 & 0.097 & r \\
59921.551 & 17.031 & 0.018 & r \\
59921.553 & 17.727 & 0.031 & i \\
59923.504 & 18.203 & 0.048 & g \\
59923.504 & 18.190 & 0.075 & g \\
59923.504 & 18.190 & 0.075 & g \\
59932.481 & 18.273 & 0.070 & g \\
59932.481 & 18.291 & 0.027 & g \\
59932.481 & 18.273 & 0.070 & g \\
59934.469 & 17.286 & 0.022 & r \\
59934.469 & 17.170 & 0.056 & r \\
59934.540 & 18.324 & 0.074 & g \\
59934.540 & 18.379 & 0.033 & g \\
59936.430 & 17.226 & 0.097 & r \\
59936.453 & 17.125 & 0.031 & r \\
59936.455 & 17.947 & 0.043 & i \\
59936.483 & 17.182 & 0.037 & r \\
59936.483 & 17.182 & 0.037 & r \\
59936.483 & 17.219 & 0.014 & r \\
59937.430 & 17.141 & 0.098 & r \\
59937.454 & 17.115 & 0.026 & r \\
59937.456 & 17.923 & 0.046 & i \\
59951.439 & 17.348 & 0.027 & r \\
59951.439 & 17.298 & 0.046 & r \\
59951.439 & 17.298 & 0.046 & r \\
59951.481 & 18.553 & 0.072 & g \\
59951.481 & 18.518 & 0.104 & g \\
59951.481 & 18.518 & 0.104 & g \\
59956.355 & 17.321 & 0.103 & r \\
59956.378 & 17.290 & 0.145 & r \\
59956.380 & 18.358 & 0.084 & i \\
59965.342 & 17.409 & 0.053 & r \\
59965.347 & 18.376 & 0.140 & i \\
59965.382 & 17.610 & 0.032 & r \\
59965.382 & 17.466 & 0.087 & r \\
59965.382 & 17.466 & 0.087 & r \\
59965.443 & 18.580 & 0.146 & g \\
59965.443 & 18.580 & 0.146 & g \\
59965.443 & 18.725 & 0.073 & g \\
59965.470 & 17.510 & 0.039 & r \\
59965.471 & 18.397 & 0.077 & i \\
59967.368 & 17.632 & 0.059 & r \\
59967.374 & 18.371 & 0.110 & i \\
59968.415 & 18.590 & 0.091 & g \\
59968.415 & 18.590 & 0.091 & g \\
59968.415 & 18.648 & 0.045 & g \\
59968.441 & 17.478 & 0.054 & r \\
59968.441 & 17.478 & 0.054 & r \\
59968.441 & 17.540 & 0.018 & r \\
59969.361 & 18.639 & 0.082 & g \\
59969.361 & 18.681 & 0.045 & g \\
59969.361 & 18.639 & 0.082 & g \\
59969.464 & 17.482 & 0.045 & r \\
59969.464 & 17.482 & 0.045 & r \\
59969.464 & 17.473 & 0.015 & r \\
59971.404 & 17.551 & 0.055 & r \\
59971.404 & 17.551 & 0.055 & r \\
59971.404 & 17.619 & 0.023 & r \\
59977.317 & 19.023 & 0.177 & g \\
59977.317 & 18.840 & 0.269 & g \\
59977.338 & 17.658 & 0.089 & r \\
59977.338 & 17.768 & 0.040 & r \\
59977.338 & 17.658 & 0.089 & r \\
59979.435 & 17.536 & 0.023 & r \\
59979.435 & 17.605 & 0.041 & r \\
59979.435 & 17.605 & 0.041 & r \\
59980.334 & 17.555 & 0.102 & r \\
59980.358 & 17.751 & 0.194 & r \\
59980.360 & 18.390 & 0.066 & i \\
59987.398 & 17.744 & 0.058 & r \\
59987.398 & 17.769 & 0.026 & r \\
59996.378 & 18.652 & 0.160 & g \\
59996.378 & 18.665 & 0.261 & g \\
60007.034 & 17.973 & 0.030 & r \\
60007.034 & 17.973 & 0.030 & r \\
60007.034 & 17.973 & 0.030 & r \\
60007.041 & 18.712 & 0.067 & g \\
60007.041 & 18.712 & 0.067 & g \\
60007.041 & 18.712 & 0.067 & g \\
60013.325 & 17.954 & 0.115 & r \\
60013.331 & 18.617 & 0.131 & i \\
60016.205 & 19.471 & 0.137 & g \\
60020.173 & 18.060 & 0.102 & r \\
60020.200 & 18.011 & 0.034 & r \\
60020.208 & 18.883 & 0.055 & i \\
60020.354 & 17.962 & 0.019 & r \\
60020.354 & 17.970 & 0.061 & r \\
60020.354 & 17.970 & 0.061 & r \\
60031.296 & 18.059 & 0.025 & r \\
60031.296 & 18.069 & 0.055 & r \\
60031.296 & 18.069 & 0.055 & r \\
60032.263 & 18.252 & 0.102 & r \\
60032.285 & 18.145 & 0.034 & r \\
60032.291 & 18.827 & 0.045 & i \\
60036.294 & 19.601 & 0.234 & g \\
60036.294 & 19.673 & 0.193 & g \\
60041.236 & 18.358 & 0.065 & r \\
60041.241 & 18.703 & 0.057 & i \\
60042.196 & 18.528 & 0.070 & i \\
60043.317 & 19.597 & 0.170 & g \\
60045.256 & 18.253 & 0.083 & r \\
60045.256 & 18.253 & 0.083 & r \\
60045.256 & 18.224 & 0.024 & r \\
60050.252 & 18.273 & 0.026 & r \\
60050.252 & 18.283 & 0.072 & r \\
60050.252 & 18.283 & 0.072 & r \\
60052.271 & 19.477 & 0.139 & g \\
60052.271 & 19.477 & 0.139 & g \\
60052.271 & 19.503 & 0.064 & g \\
60052.275 & 18.307 & 0.070 & r \\
60052.275 & 18.307 & 0.070 & r \\
60052.275 & 18.306 & 0.027 & r \\
60053.391 & 18.384 & 0.073 & r \\
60054.254 & 19.519 & 0.146 & g \\
60054.254 & 19.521 & 0.074 & g \\
60054.254 & 19.519 & 0.146 & g \\
60056.169 & 18.411 & 0.031 & r \\
60056.169 & 18.410 & 0.072 & r \\
60056.169 & 18.409 & 0.072 & r \\
60056.211 & 19.637 & 0.076 & g \\
60056.211 & 19.611 & 0.173 & g \\
60056.211 & 19.611 & 0.173 & g \\
60058.232 & 18.347 & 0.067 & r \\
60058.232 & 18.347 & 0.067 & r \\
60058.232 & 18.354 & 0.035 & r \\
60058.319 & 19.562 & 0.081 & g \\
60058.319 & 19.539 & 0.143 & g \\
60058.319 & 19.539 & 0.143 & g \\
60060.305 & 18.375 & 0.038 & r \\
60060.305 & 18.364 & 0.067 & r \\
60060.305 & 18.364 & 0.067 & r \\
60062.194 & 18.309 & 0.075 & r \\
60062.194 & 18.308 & 0.075 & r \\
60062.194 & 18.272 & 0.038 & r \\
60062.219 & 19.572 & 0.109 & g \\
60062.219 & 19.554 & 0.185 & g \\
60062.219 & 19.554 & 0.185 & g \\
60064.276 & 18.524 & 0.103 & r \\
60064.276 & 18.524 & 0.103 & r \\
60064.276 & 18.514 & 0.053 & r \\
60073.276 & 19.832 & 0.135 & g \\
60073.276 & 19.857 & 0.257 & g \\
60077.211 & 18.551 & 0.074 & r \\
60077.211 & 18.542 & 0.034 & r \\
60077.211 & 18.551 & 0.074 & r \\
60078.296 & 18.624 & 0.048 & r \\
60079.600 & 18.967 & 0.074 & o \\
60081.233 & 18.601 & 0.048 & r \\
60081.233 & 18.587 & 0.106 & r \\
60081.233 & 18.587 & 0.106 & r \\
60083.219 & 18.532 & 0.031 & r \\
60083.219 & 18.582 & 0.080 & r \\
60083.219 & 18.582 & 0.080 & r \\
60085.229 & 20.127 & 0.117 & g \\
60085.570 & 18.636 & 0.049 & o \\
60088.190 & 18.626 & 0.031 & r \\
60088.190 & 18.667 & 0.069 & r \\
60088.190 & 18.667 & 0.069 & r \\
60088.290 & 20.005 & 0.126 & g \\
60091.590 & 19.017 & 0.080 & o \\
60093.550 & 18.897 & 0.071 & o \\
60095.560 & 18.806 & 0.063 & o \\
60097.235 & 18.808 & 0.154 & r \\
60097.235 & 18.808 & 0.154 & r \\
60103.190 & 18.837 & 0.079 & r \\
60103.190 & 18.837 & 0.079 & r \\
60103.560 & 18.691 & 0.071 & o \\
60105.235 & 18.884 & 0.113 & r \\
60105.235 & 18.884 & 0.113 & r \\
60105.510 & 18.453 & 0.090 & o \\
60107.530 & 18.535 & 0.084 & o \\
\bottomrule
\end{tabular}
\end{table}
